Parameterized Approximation for Maximum Weight Independent Set of Rectangles and Segments

In the Maximum Weight Independent Set of Rectangles problem (MWISR) we are given a weighted set of $n$ axis-parallel rectangles in the plane. The task is to find a subset of pairwise non-overlapping rectangles with the maximum possible total weight. This problem is NP-hard and the best-known polynomial-time approximation algorithm, due to by Chalermsook and Walczak (SODA 2021), achieves approximation factor $O(\log\log n )$. While in the unweighted setting, constant factor approximation algorithms are known, due to Mitchell (FOCS 2021) and to G\'alvez et al. (SODA 2022), it remains open to extend these techniques to the weighted setting. In this paper, we consider MWISR through the lens of parameterized approximation. Grandoni et al. (ESA 2019) gave a $(1-\epsilon)$-approximation algorithm with running time $k^{O(k/\epsilon^8)} n^{O(1/\epsilon^8)}$ time, where $k$ is the number of rectangles in an optimum solution. Unfortunately, their algorithm works only in the unweighted setting and they left it as an open problem to give a parameterized approximation scheme in the weighted setting. Our contribution is a partial answer to the open question of Grandoni et al. (ESA 2019). We give a parameterized approximation algorithm for MWISR that given a parameter $k$, finds a set of non-overlapping rectangles of weight at least $(1-\epsilon) \text{opt}_k$ in $2^{O(k \log(k/\epsilon))} n^{O(1/\epsilon)}$ time, where $\text{opt}_k$ is the maximum weight of a solution of cardinality at most $k$. Note that thus, our algorithm may return a solution consisting of more than $k$ rectangles. To complement this apparent weakness, we also propose a parameterized approximation scheme with running time $2^{O(k^2 \log(k/\epsilon))} n^{O(1)}$ that finds a solution with cardinality at most $k$ and total weight at least $(1-\epsilon)\text{opt}_k$ for the special case of axis-parallel segments.

==> Makefile <==
SOURCES := $(shell find $(SOURCEDIR) -name '*.tex')

all: main.pdf

main.pdf: $(SOURCES) main.bbl 
	pdflatex main.tex
	pdflatex main.tex

main.aux: $(SOURCES)
	pdflatex main.tex

main.bbl: bib.bib main.aux
	bibtex main

clean:
	rm -f img/*.log img/*.aux 
	rm -f *~ *.log *.out *.aux *.blg *.bbl *.gz

distclean: clean
	rm -f main.pdf

tar: clean
	bash -c "cd ..; tar -czf ${BASE}.tar.gz ${BASE}/*; mv ${BASE}.tar.gz ${BASE}"

spell:
	@for i in `find . -name "*.tex"` ; do \
		echo "------------ $$i --------------" ; \
		aspell list --lang=en --mode=tex --dont-tex-check-comments --personal=./blue-slownik.txt < $$i | sort | uniq ; \
done

diff:
	mkdir /tmp/cut-and-count-diff/
	python2 ~/latex-flatten.py main.tex /tmp/cut-and-count-diff/test.tex
	python2 ~/latex-flatten.py /tmp/cut-and-count-diff/test.tex /tmp/cut-and-count-diff/test2.tex
	python2 ~/latex-flatten.py /tmp/cut-and-count-diff/test2.tex /tmp/cut-and-count-diff/d2.tex
	git checkout $(branch-id)
	python2 ~/latex-flatten.py main.tex /tmp/cut-and-count-diff/test.tex
	python2 ~/latex-flatten.py /tmp/cut-and-count-diff/test.tex /tmp/cut-and-count-diff/test2.tex
	python2 ~/latex-flatten.py /tmp/cut-and-count-diff/test2.tex /tmp/cut-and-count-diff/d1.tex
	latexdiff /tmp/cut-and-count-diff/d1.tex /tmp/cut-and-count-diff/d2.tex > /tmp/cut-and-count-diff/diff.tex
	pdflatex /tmp/cut-and-count-diff/diff.tex
	git checkout master


==> chapters/conclusion.tex <==
\section{Conclusion and Open Problems}

In this paper we consider parameterized approximation schemes for finding maximum weight
independent sets of axis-parallel rectangles and segments parameterized by
the cardinality of the solution $k \in \nat$. We demonstrated that one can find an
independent set of weight $\ge (1-\eps)\omega(\opt_k)$ in parameterized time.
This partially answers an open question posed in Grandoni et al.~\cite{esa19}. A
weakness of our method is that our algorithm can return a set of unbounded
cardinality.

To address this issue, we show that this can be achieved in the restricted
setting of weighted axis-parallel segments. For this problem we give a
parameterized approximation scheme that returns an independent set of cardinality
$\le k$ and weight $\ge (1-\eps)\omega(\opt_k)$. A natural open question is to
show that this is also possible for rectangles.

